Succinct Explanations With Cascading Decision Trees

The decision tree is one of the most popular and classical machine learning models from the 1980s. However, in many practical applications, decision trees tend to generate decision paths with excessive depth. Long decision paths often cause overfitting problems, and make models difficult to interpret. With longer decision paths, inference is also more likely to fail when the data contain missing values. In this work, we propose a new tree model called Cascading Decision Trees to alleviate this problem. The key insight of Cascading Decision Trees is to separate the decision path and the explanation path. Our experiments show that on average, Cascading Decision Trees generate 63.38% shorter explanation paths, avoiding overfitting and thus achieve higher test accuracy. We also empirically demonstrate that Cascading Decision Trees have advantages in the robustness against missing values.

==> secs/future.tex <==
\section{Future Work}


%Classic decision tree
%Cascasding
\para{Missing Value Handling}
Missing values are a widespread problem in classification.
Especially in medical domains, missing values are unfortunately unavoidable~\cite{Danilo15medicalmissing}.
Running studies with no missing value results in a smaller sample size with less statistical significance.

%Classic decision tree
The decision rule in classic decision trees is constructed by the traverse of each decision along the decision path.
As a result, when the algorithm encounters a missing value in one of its decision nodes, it is forced to stop and is unable to provide a classification.
Compared with the classic decision trees algorithm, cascading decision trees algorithm has better tolerance to the missing value in the testing sample.

For instance, with the same dataset shown in $\S$\ref{sec:motivation}, suppose a new sample comes with a \texttt{False} in \texttt{Feature 1} and \texttt{Feature 3}, a \texttt{True} in \texttt{Feature 4} but with a missing value in \texttt{Feature 3}. 
This sample will be classified as \texttt{Positive} with a root cause of \texttt{True} in \texttt{Feature 4}.
However, using the classic decision trees algorithm results in an early stop after the split in the depth two, and fails to provide the correct prediction \texttt{Positive}.
Future studies will focus on quantifying the ability of the cascading decision trees algorithm on missing value handling requires real-world medical data.

%\para{Short Circuiting}

%\para{Missing Value Handling}
